SpeechVerse: A Large-scale Generalizable Audio Language Model

Large language models (LLMs) have shown incredible proficiency in performing tasks that require semantic understanding of natural language instructions. Recently, many works have further expanded this capability to perceive multimodal audio and text inputs, but their capabilities are often limited to specific fine-tuned tasks such as automatic speech recognition and translation. We therefore develop SpeechVerse, a robust multi-task training and curriculum learning framework that combines pre-trained speech and text foundation models via a small set of learnable parameters, while keeping the pre-trained models frozen during training. The models are instruction finetuned using continuous latent representations extracted from the speech foundation model to achieve optimal zero-shot performance on a diverse range of speech processing tasks using natural language instructions. We perform extensive benchmarking that includes comparing our model performance against traditional baselines across several datasets and tasks. Furthermore, we evaluate the model's capability for generalized instruction following by testing on out-of-domain datasets, novel prompts, and unseen tasks. Our empirical experiments reveal that our multi-task SpeechVerse model is even superior to conventional task-specific baselines on 9 out of the 11 tasks.

==> 401.results.tex <==

\section{Results [WIP, will be revised]}

\subsection{Evaluation of SpeechVerse models}
\label{subsec:speechverse_performance}

We evaluate SpeechVerse on 11 unique tasks spanning multiple domains and datasets. We first evaluate SpeechVerse's core speech understanding capability through ASR benchmarks. We then evaluate more complex spoken language understanding (SLU) tasks and paralinguistic speech tasks in Tables \ref{tab:pipelined_tasks} and \ref{tab:non_pipelined_tasks} respectively. Finally, we compare our model performance against SOTA models on five representative tasks. 

\subsubsection{Performance on ASR and SLU tasks} 

First, we evaluate the performance of SpeechVerse models on four public ASR benchmark datasets namely \textit{libri-test-clean}, \textit{libri-test-other}, \textit{Voxpopuli} and \textit{CommonVoice}. The WER numbers for each of these datasets are reported in Table \ref{tab:pipelined_tasks}. When comparing our task-specific pretrained ASR model, which also serves as the initialization for multi-task finetuning, to Whisper-large-v2, our model achieves better performance on three out of the four ASR benchmarks. Both multi-task models perform similarly to Whisper across the ASR benchmarks.

When it comes to SLU tasks, a frequent question posed is if an end-to-end model can outperform a cascaded pipeline that transcribes speech via ASR and then feeds it to a language model. To investigate this, we conducted experiments on five semantic understanding tasks using the same foundation models as SpeechVerse. The text foundation model was further fine-tuned on data from the five SLU tasks separately, as we found the zero-shot performance of Flan-T5 on these benchmark test sets to be quite poor. We also report performance when feeding ground-truth transcripts into the fine-tuned LLM, to provide upper bound results. On 4 of the 5 tasks, excluding Keyword Extraction, the end-to-end trained models outperform the cascaded pipeline. When comparing the multi-task models to the task-specific SpeechVerse models, there is a minor degradation in performance, but the difference is not substantial.

\subsubsection{Performance on paralinguistic tasks} 

The results in Table \ref{tab:non_pipelined_tasks} demonstrate clear improvements in performance on various paralinguistic speech processing tasks when using multi-task learning compared to fine-tuning the WavLM model independently for each task. Specifically, the SpeechVerse model trained with multitask learning using Best-RQ audio encoder (Multitask-BRQ) achieves gains over the baseline WavLM model of 4.8\% absolute on emotion recognition, 6.6\% on audio sentiment classification, and 2.5\% on accent classification. More modest gains are seen with the SpeechVerse model trained using multitask learning with WavLM encoder (Multitask-WLM), showing the benefits of the unified representation. Overall, multi-task learning provides noticeable improvements in model generalization and effectiveness across a diverse set of speech analysis tasks compared to task-specific fine-tuning of the baseline WavLM model. The results highlight the advantages of learning shared representations across related tasks using multi-task learning techniques.

%Table \ref{tab:non_pipelined_tasks} reports performance on five paralinguistic classification tasks, comparing SpeechVerse to conventional baselines using a \textit{WavLM-large} speech encoder fine-tuned with a softmax classifier. Overall, SpeechVerse matches or exceeds the WavLM baseline across all tasks. Among the multitask models, combining representations from all layers significantly outperforms using just the top layer. Additionally, the multitask SpeechVerse models perform on par with or better than the task-specific SpeechVerse variants.

% \subsubsection{Comparison against SOTA models} Table \ref{tab:sota_benchmarking} benchmarks SpeechVerse against state-of-the-art models on five diverse tasks: automatic speech recognition (ASR), automatic speech translation (AST), intent classification (IC), slot filling (SF), and emotion recognition (ER). Across these tasks, SpeechVerse demonstrates competitive or superior performance compared to prior specialized models. 

\subsubsection{Comparison against prior SOTA models}
\label{app:sota_performance}

\input{table-zero-shot-results}

Table \ref{tab:sota_benchmarking} benchmarks SpeechVerse models against state-of-the-art (SOTA) models on five diverse tasks: automatic speech recognition (ASR), speech translation (ST), intent classification (IC), slot filling (SF), and emotion recognition (ER). Across these tasks, SpeechVerse demonstrates competitive or superior performance compared to prior specialized models. When comparing our task-specific pretrained ASR model, which also serves as the initialization for multi-task finetuning, to Whisper ASR, our model achieves slightly better performance on average. However, the multitask model (\textit{Multitask-WLM}) performed similarly to Whisper across three out of the four test sets. When evaluating on speech translation across three language pairs, the task-specialized SpeechVerse model surpassed SeamlessM4T on two pairs, while the multi-task SpeechVerse model achieved competitive performance compared to prior work on average. Both models did not perform well on English to Romanian pair. The overall performance of the SpeechVerse models on speech translation is heavily limited by the capabilities of the underlying language model FlanT5. The speech translation capabilities cannot exceed the translation quality provided by FlanT5 as the base language model. To evaluate SpeechVerse on spoken language understanding tasks like intent classification (IC) and slot filling (SF), we retrained the task-specialized SpeechVerse model by incorporating all 69 intents (both seen and unseen) as well as all slots. This allowed us to compare SpeechVerse to prior work on the complete intent and slot sets. Our SpeechVerse model achieved competitive performance to the previous SOTA (\textit{PF-hbt-large}) on slot filling, but was significantly behind on intent classification with 5\% lower absolute accuracy. However, SpeechVerse outperformed the same SOTA model (\textit{Frozen-hbt-large}) by 10\% when the encoder weights were frozen during fine-tuning. To further analyze the gap to prior state-of-the-art, we conducted an experiment allowing the encoder weights to be tunable during fine-tuning. This achieved 89.5\% accuracy, matching the prior SOTA. This suggests the intent classification performance can overfit to the specific acoustic conditions of the SLURP dataset when full fine-tuning is performed. The SpeechVerse model that was trained end-to-end specifically for the task of emotion recognition achieved an 8\% absolute improvement in unweighted average recall over the previous state-of-the-art model (\textit{w2v2-L-robust}). In contrast, the multitask SpeechVerse model performed 3\% better than the prior state-of-the-art. However, one key difference is that the previous SOTA work trained on the MSP-Podcast 1.7 dataset, while we used version 1.11 for training. The test set version remained the same between the two approaches. Overall, the SpeechVerse model demonstrated competitive performance compared to prior specialized models in some cases when evaluated across the various tasks.





\subsection{Generalization Across Instructions}
\label{subsec:generalization}

To comprehensively evaluate the model's ability to generalize instruction following, we tested performance on three types of instructions: 1) new instructions with different wording and context, 
2) known task instructions tested on out-of-domain datasets requiring adaptation to new contexts, and 3) instructions for entirely new tasks not seen during training. 

%\pra{is average length of prompt similar to that in training?} 

\subsubsection{Measuring prompts performance}
\label{ssub:prompts_performance}

\begin{table}[t]
\caption{Generalization to unseen prompts: The performance of each task is assessed on three different prompts, out of which, two are unseen during training.}
\label{tab:unseen_prompts}
\centering
\footnotesize
%\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\makecell{\textbf{Prompt} \\ \textbf{(Unseen)}}}  & \multicolumn{2}{c}{\textbf{Performance}}  \\
\cmidrule{4-5}
& & & \textbf{Metric} & \textbf{Results} \\
\midrule
\multirow{3}{*}{ASR} & \multirow{3}{*}{Voxpopuli} & P1 (\xmark) & \multirow{3}{*}{WER$\downarrow$} & 6.5 \\
 & & P2 (\cmark) & & 6.6 \\
 & & P3 (\cmark) & & 6.6 \\
 \midrule
 \multirow{3}{*}{AST} & \multirow{3}{*}{\makecell{CoVoST \\ EN$\rightarrow$DE}} & P1 (\xmark) & \multirow{3}{*}{BLEU$\uparrow$} & 25.1 \\
 & & P2 (\cmark) & & 25.3 \\
 & & P3 (\cmark) & & 25.0 \\
 \midrule
 \multirow{3}{*}{AC} & \multirow{3}{*}{MCV} & P1 (\xmark) & \multirow{2}{*}{F1$\uparrow$} & 65.1 \\
 & & P2 (\cmark) & & 65.0 \\
 & & P3 (\cmark) & & 65.3 \\
\bottomrule
\end{tabular}
%}
\end{table}

To evaluate the effect of different prompts on core task performance, we tested the selected model on two seen prompts and one novel prompt for each of three tasks: speech recognition, translation, and emotion recognition. The seen prompts were taken directly from the training data, while the novel prompts required the same core capability but with different wording and context. The model showed similar performance across prompts for each task. For speech recognition, measured by word error rate (WER), there was a difference of only 0.1-0.2 between the seen and novel prompts. Translation performance, measured by BLEU score, varied by up to 0.2 across prompts. For emotion recognition, F1 scores differed by 0.1 or less across the three prompts. %\pra{Is this in line with prior works on prompt tuning?}

%\xing{Do we compare with a baseline system that is only trained with one prompt per task?} 
These small differences indicate the model has generalized its core capabilities well and is not strongly dependent on the specific wording or context of the prompts. The similar WER, BLEU, and F1 scores across seen and novel prompts for each task demonstrate good generalization beyond the training data. While prompt engineering remains important for optimal performance, these results suggest that the model has learned robust task-specific skills that transfer across varied inputs requiring the same core capability. Further analysis across a wider range of prompts and tasks would strengthen these conclusions about the generalization abilities of the model but left for future work.

\subsubsection{Performance on out-of-domain (OOD) datasets}
\label{ssub:unseen_domains}

\iffalse
\begin{table}[t]
\caption{Generalization to unseen domains: The performance of each task is assessed on out-of-domain (OOD) datasets.}
\label{tab:unseen_prompts}
\centering
\footnotesize
%\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
\textbf{Task} & \textbf{Dataset} & \textbf{Metric} & \textbf{Task-FT} & \textbf{Multitask} \\
\midrule
\multirow{3}{*}{ASR} & WSJ & \multirow{3}{*}{WER} & - & - \\
 & CORAAL & & - & - \\
 & Chime & & - & - \\
 \midrule
 \multirow{2}{*}{AC} & GMU & \multirow{2}{*}{UAR} & - & - \\
 & CORAAL & & - & - \\
\bottomrule
\end{tabular}
%}
\end{table}
\fi

%\pra{Did we ensure that there is no task and data leakage?}

To evaluate generalization of instruction following, we tested both a multi-task model and task-specific models on out-of-domain datasets containing novel contexts. The instructions came from known tasks the models were trained on, but required adaptation to new situations and domains. The multi-task model showed higher accuracy on the out-of-domain data compared to the task-specific models. The consistent performance of the multi-task model despite distributional shift demonstrates the robustness of its core instruction following skills. Rather than overfitting to the training domain, the multi-task learning approach enabled the model to learn more flexible capabilities in instruction comprehension and execution that better transfer to new contexts. The superior performance of the multi-task model on out-of-domain data provides key evidence for improved generalization of core instruction following abilities through multi-task training.

\subsubsection{Performance on unseen tasks}
\label{ssub:unseen_tasks}

\iffalse
\begin{table}[h]
\caption{Results on Speech dialogue dataset with classification into 8 different domains. DC: Domain Classification;}
\label{tab:domain_classification}
\centering
\footnotesize
%\resizebox{0.49\textwidth}{!}{
\begin{tabular}{cccc}
\toprule
\textbf{Task} & \textbf{Input} & \textbf{Model} & \makecell{\textbf{Average} \\ \textbf{Recall}} \\
\midrule
\multirow{2}{*}{DC} & Text & Flan-T5 & 54.1 \\
 & Audio & SpeechVerse & 56.1 \\
\bottomrule
\end{tabular}
%}
\end{table}
\fi

To further assess generalization, we evaluated the multi-task model on entirely novel tasks not seen during training. The model was given instructions describing new tasks that required adapting its capabilities to new contexts. In Table \ref{tab:domain_classification}, we provide results on domain classification task which is an unseen task during training. Results showed the multi-task model was able to perform domain classification with reasonable accuracy, without any task-specific fine-tuning. Table \fixme{TBD} provides examples of the model's responses to instructions for novel, unseen tasks. These qualitative examples demonstrate the model's ability to interpret and complete new tasks it was not trained on, complementing the quantitative results. The ability to follow instructions for new, unfamiliar tasks demonstrates that the model learned a generalized instruction following skill, rather than just memorizing associations for the trained tasks. Testing on unseen tasks provides additional evidence that the multi-task training approach improved generalization and flexibility in core instruction following abilities.

%Overall, the model performed quite well across all three categories of  instructions. These robust results across instructions with differing wording, domain, and task demonstrate the model has learned flexible core skills for interpreting and executing novel instructions. The model has not simply memorized input-output pairings but rather developed generalized capabilities in comprehension and following instructions in varied contexts. Testing on out-of-domain data and unseen tasks provides stronger evidence for the model's ability to generalize instruction following beyond its training.

%\subsection{Decoding strategies}


%\subsubsection{Study on constrained decoding}
%\label{ssub:constrained_decoding}

\begin{table*}[t]
\caption{Results on three unseen tasks with (w/) and without (w/o) constrained decoding. `-' indicates that constrained decoding is not possible in that setting.}
\label{tab:constrained_decoding}
\vspace{-2mm}
\centering
\footnotesize
%\resizebox{0.49\textwidth}{!}{
% \begin{tabular}{cccccc}
% \toprule
% \multirow{3}{*}{\textbf{Task}} & \multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\makecell{\textbf{\# of} \\ \textbf{Classes}}} & \multirow{3}{*}{\textbf{Metric}} & \multicolumn{2}{c}{\makecell{\textbf{Constrained} \\ \textbf{Decoding}}} \\
% \cmidrule{5-6}
% & & & & \textbf{w/o} & \textbf{w/} \\
% \midrule
% \multirow{2}{*}{IC} & SLURP & 10 & \multirow{2}{*}{ACC} & 52.4 & 60.5 \\
%  & SNIPS & 15 &  & 22.1 & 46.3 \\
% \multirow{2}{*}{SF} & SLURP & 10 & \multirow{2}{*}{F1} & 95.5 & 96.5 \\
%  & SNIPS & 15 &  & 37.5 & 43.3 \\
% ER & MSP & 4 & UAR & 65.1 & 67.5 \\
% \bottomrule
% \end{tabular}
%}
\begin{tabular}{llccc}
\toprule
\multirow{2}{*}{Model}                         & \multirow{2}{*}{Training} & IC (ACC$\uparrow$) & ST (BLEU$\uparrow$) & DC (ACC$\uparrow$) \\ \cmidrule(l){3-5} 
                                               &                           & SNIPS              & EN$\rightarrow$ES   & Internal           \\ \midrule
SpeechVerse ASR $\rightarrow$ LLM              & LLM-FT                    & 86.2               & 14.3                & 48.3               \\
SpeechVerse E2E-SLM (w/o Constrained Decoding) & Multitask-Top             & 61.0               & 15.8                & 56.9               \\
SpeechVerse E2E-SLM (w/ Constrained Decoding)  & Multitask-Top             & 75.9               & -                   & 59.0               \\ \midrule
GT $\rightarrow$ LLM                           & LLM-FT                    & 91.4               & 16.4                & 51.0               \\ \bottomrule
\end{tabular}
\end{table*}

%The work in \citet{willard2023efficient} introduced a model-agnostic technique to enforce domain-specific knowledge and constraints during text generation. Building on this prior approach, we have explored applying decoding constraints to our SpeechVerse models to improve their performance on text classification tasks like intent detection and slot filling. Rather than allowing the model to generate freely in response to a prompt, the decoding is restricted to output from a predefined vocabulary of class names. For example, in an intent classification task, the model would be constrained to only generate intent labels such as ``\textit{calendar\_set}'', ``\textit{email\_query}'', or ``\textit{play\_music}''. By limiting the output space, the model is more likely to produce the desired class label rather than unrelated text. %Experiments on both intent classification and slot filling tasks have shown consistent gains in accuracy from employing constrained decoding compared to standard free-form decoding (See Table \ref{tab:constrained_decoding}).

%The results in Table \ref{tab:constrained_decoding} demonstrate clear improvements across three text classification tasks when applying constrained decoding during inference. For intent classification (IC), constrained decoding improved accuracy substantially on both the SLURP and SNIPS datasets, with gains of 8.1\% and 24.2\% respectively. For slot filling (SF), constrained decoding yielded F1 score increases on SLURP and SNIPS as well, though the gains were more modest at 1\% and 5.8\%. Finally, for emotion recognition (ER) using the MSP dataset, the use of constraints during decoding improved unweighted average recall by 2.4\%. Overall, constrained decoding consistently enhanced model performance on unseen classes across tasks and datasets compared to unconstrained inference. By enforcing domain-specific knowledge and constraints during decoding, the model outputs can be guided to better match the desired classifications. These results highlight the potential of constrained decoding to improve generalization of large pre-trained language models to new distributions and tasks.



==> ack.tex <==
\section*{Acknowledgements}

\fixme{TBD.}

